Towards Effective Authorship Attribution: Integrating Class-Incremental Learning

AA is the process of attributing an unidentified document to its true author from a predefined group of known candidates, each possessing multiple samples. The nature of AA necessitates accommodating emerging new authors, as each individual must be considered unique. This uniqueness can be attributed to various factors, including their stylistic preferences, areas of expertise, gender, cultural background, and other personal characteristics that influence their writing. These diverse attributes contribute to the distinctiveness of each author, making it essential for AA systems to recognize and account for these variations. However, current AA benchmarks commonly overlook this uniqueness and frame the problem as a closed-world classification, assuming a fixed number of authors throughout the system's lifespan and neglecting the inclusion of emerging new authors. This oversight renders the majority of existing approaches ineffective for real-world applications of AA, where continuous learning is essential. These inefficiencies manifest as current models either resist learning new authors or experience catastrophic forgetting, where the introduction of new data causes the models to lose previously acquired knowledge. To address these inefficiencies, we propose redefining AA as CIL, where new authors are introduced incrementally after the initial training phase, allowing the system to adapt and learn continuously. To achieve this, we briefly examine subsequent CIL approaches introduced in other domains. Moreover, we have adopted several well-known CIL methods, along with an examination of their strengths and weaknesses in the context of AA. Additionally, we outline potential future directions for advancing CIL AA systems. As a result, our paper can serve as a starting point for evolving AA systems from closed-world models to continual learning through CIL paradigms.

==> documents/CIL-Taxonomy.tex <==
% \subsection{CIL Taxonomy}
% CIL has recently gained increasing attention across various domains, including image classification, face recognition, and vehicle detection \cite{yan2021dynamically, zhou2022model, jodelet2023class, hu2023dense, madhavan2021incremental, li2022few}. Its popularity has surged primarily due to the widespread adoption of large-scale models like GPT-2, where retraining the entire model for new classes becomes impractical. Additionally, CIL proves beneficial in scenarios where the privacy of data is paramount \cite{chamikara2018efficient}, necessitating models that do not retain training data. Despite numerous attempts in the literature to categorize existing approaches to CIL, a unified taxonomy remains elusive \cite{masana2022class, zhou2023deep, mai2022online, tian2024survey}. This challenge arises because existing techniques often overlap, making non-overlapping categorization difficult to achieve. Therefore, we offer our brief and high-level taxonomy of existing CIL approaches based on their level of ease in integrating with existing AA approaches, primarily leveraging pre-trained models. In general, CIL deals with the "stability-plasticity" dilemma \cite{mermillod2013stability}, where the learner must balance the ability to retain acquired knowledge (stability) with the capacity to learn new tasks (plasticity). An extreme case of plasticity can lead to catastrophic forgetting \cite{french1999catastrophic, goodfellow2013empirical, mccloskey1989catastrophic}, where the model focuses solely on learning new data, resulting in the loss of previously acquired information. Consequently, existing approaches aim to find the optimal balance through various perspectives, as follows: \newline

CIL has recently gained increasing attention across various domains, including image classification, face recognition, and vehicle detection \cite{yan2021dynamically, zhou2022model, jodelet2023class, hu2023dense, madhavan2021incremental, li2022few}. Its popularity has surged primarily due to the widespread adoption of large-scale models like GPT-2, where retraining the entire model for new classes becomes impractical. Additionally, CIL proves beneficial in scenarios where the privacy of data is paramount \cite{chamikara2018efficient}, necessitating models that do not retain training data. Despite numerous attempts in the literature to categorize existing approaches to CIL, a unified taxonomy remains elusive \cite{masana2022class, zhou2023deep, mai2022online, tian2024survey}. This challenge arises because existing techniques often overlap, making non-overlapping categorization difficult to achieve. Therefore, we offer our brief and high-level taxonomy of existing CIL approaches based on their level of ease in integrating with existing AA approaches. In general, CIL deals with the "stability-plasticity" dilemma \cite{mermillod2013stability}, where the learner must balance the ability to retain acquired knowledge (stability) with the capacity to learn new tasks (plasticity). An extreme case of plasticity can lead to catastrophic forgetting \cite{french1999catastrophic, mccloskey1989catastrophic}, where the model focuses solely on learning new data, resulting in the loss of previously acquired information. Consequently, existing approaches aim to find the optimal balance through various perspectives, as follows: \newline



% \subsubsection{Replay} is a straightforward approach within CIL strategies that directly address catastrophic forgetting \cite{wu2019large, castro2018end}, especially prevalent in fine-tuning scenarios. This method involves preserving acquired knowledge by retaining a subset of exemplars for model rehearsal in subsequent sessions, which may originate from previous sessions or be synthetically generated through models such as Generative Adversarial Networks (GANs) or low-dimensional transformed representations \cite{xiang2019incremental, shin2017continual}. Exemplar sampling strategies within replay methods vary widely. Random sampling, despite its computational efficiency, has demonstrated effectiveness \cite{chaudhry2018riemannian}. Alternatively, more refined strategies select exemplars that are most informative, such as those near decision boundaries (hard samples) or with higher entropy derived from softmax outputs \cite{chaudhry2018riemannian}. To manage memory efficiently, two primary approaches have been proposed: fixed memory and dynamic memory. Fixed memory sizes offer simplicity but entail overhead in adding and removing exemplars, as well as operational costs associated with these tasks. In contrast, dynamic memory allows seamless addition of new examples but requires more storage as it grows linearly with the introduction of new data \cite{chaudhry2018riemannian}. Beyond its straightforward implementation, replay demonstrates potential benefits, particularly when integrated with fine-tuning and alignment, which have shown numerous successes in literature. However, challenges include the risk of overfitting due to imbalances in the number of examples from previous and current classes, as well as the complexity of fine-tuning large models, necessitating a substantial number of samples in incremental sessions, which may not always be feasible, such as in FSCIL. Furthermore, optimizing the parameters to suit specific datasets remains a variable task. \newline


\subsubsection{Replay} This method involves preserving acquired knowledge by retaining a subset of exemplars for model rehearsal in subsequent sessions, which may originate from previous sessions or be synthetically generated through models such as Generative Adversarial Networks (GANs) or low-dimensional transformed representations \cite{xiang2019incremental, shin2017continual}. Exemplar sampling strategies within replay methods vary widely. Random sampling, despite its computational efficiency, has demonstrated effectiveness \cite{chaudhry2018riemannian}. Alternatively, more refined strategies select exemplars that are most informative, such as those near decision boundaries (hard samples) or with higher entropy derived from softmax outputs \cite{chaudhry2018riemannian}. To manage memory efficiently, two primary approaches have been proposed: fixed memory and dynamic memory. Fixed memory sizes offer simplicity but entail overhead in adding and removing exemplars, as well as operational costs associated with these tasks. In contrast, dynamic memory allows seamless addition of new examples but requires more storage as it grows linearly with the introduction of new data \cite{chaudhry2018riemannian}. Beyond its straightforward implementation, replay demonstrates potential benefits, particularly when integrated with fine-tuning and alignment, which have shown numerous successes in literature. However, challenges include the risk of overfitting due to imbalances in the number of examples from previous and current classes, as well as the complexity of fine-tuning large models. \newline


% \subsubsection{Sequential Adaptation} This strategy is based on the concept of sequential learning, where it is assumed that the learner in session \( t-1 \) performed well in the previous classes and can transfer, adjust, or correct the learner in session \( t \). This strategy originally emerged in task-incremental learning, a specific problem in incremental learning where the tasks differ across sessions, unlike in class-incremental learning where the classes differ. To achieve this, numerous approaches have been proposed, which can be further categorized into \textit{parameter regularization}, \textit{data regularization}, and \textit{knowledge distillation}.\newline

\subsubsection{Sequential Adaptation} This strategy is based on the concept of sequential learning, where it is assumed that the learner in session \( t-1 \) performed well in the previous classes and can transfer, adjust, or correct the learner in session \( t \). To achieve this, numerous approaches have been proposed, which can be further categorized into \textit{parameter regularization}, \textit{data regularization}, and \textit{knowledge distillation}.\newline



\noindent\textbf{Parameter Regularization} This concept relies on two key assumptions: (1) the contributions of the parameters in the CIL model are not equal for classification tasks, and (2) the model's parameters are independent of each other. The algorithm begins by determining the importance of each model parameter in classifying each author in session \( t-1 \). A copy of the learner parameters from this session is then obtained and frozen for the next session. When new authors are introduced to the model, it updates its parameters. The algorithm compares the current parameters to the frozen parameters from the previous session, and penalizes the model for significant differences in parameters that were deemed important. Moreover, the second assumption of parameter independence ensures computational feasibility, given the typically large number of model parameters. To implement this, an additional loss term is added to the main loss to penalize significant changes in important parameters:
{\small
\begin{equation}
L_{\text{reg}} = \frac{1}{2} \sum_{i=1}^{|\theta^{t-1}|} \Omega_i (\theta^{t-1}_i - \theta^t_i)^2
\end{equation}
}
Here, $\theta^t_i$ is the $i$th weight currently being trained, $\theta^{t-1}_i$ is its value after training in session $t-1$, $|\theta^{t-1}|$ is the number of weights, and $\Omega_i$ represents the importance of the $i$th parameter. Different methods have been proposed to determine $\Omega$ \cite{kirkpatrick2017overcoming, liu2018rotate}.\newline







\noindent\textbf{Data Regularization} 

Assume that the learner in session  \( t-1 \) correctly classified the authors seen in that session, given that the model has access to the complete documents of the authors. By transferring the learner and some documents from this session to session \( t \), these components can be sufficient for the new learner to adjust its behavior, allowing it to continue learning while exhibiting the similar performance as the previous frozen model. For instance, \cite{lopez2017gradient} introduced the following regularization term into the main loss function:

{\small
\begin{equation}
\sum_{(x_{j},y_{j}) \in D_{0}^{t-1}} \ell(f_{\theta}(x_{j}),y_{j}) \leq \sum_{(x_{j},y_{j}) \in D_{0}^{t-1}} \ell(f_{\theta}^{t-1}(x_{j}),y_{j})
\end{equation}
}
Here, $f_{\theta}$ denotes the model with parameters $\theta$, and $f_{\theta}^{t-1}$ represents the model after training the last session $S_{t-1}$. $D_{t}$ represents the current session data while $D_{0}^{t-1}$ denotes an exemplar set derived from sessions $D_{0}$ up to $D_{t-1}$. The above loss term encourages the current model to update with the restriction that the loss obtained from the current model does not exceed the loss of the previous model on the transferred exemplar set. \newline



\noindent\textbf{Knowledge Distillation} is defined as the process of transferring knowledge from a larger, more complex model (referred to as the teacher) to a smaller, simpler model (referred to as the student) \cite{hinton2015distilling}. This approach can be seamlessly adapted for CIL by treating the model \( f^{t-1} \) as the teacher and the current model \( f^t \) as the student. In this transfer process, the student model can undergo logit distillation, where it is encouraged to produce output probabilities that align with those of the teacher model \cite{rebuffi2017icarl, li2017learning}. Alternatively, for feature distillation, the objective is to produce similar feature representations \cite{hou2019learning, lu2022augmented}.\newline

In general, the primary advantage of Sequential Adaptation approaches lies in their ease of integration with existing models, particularly for AA models that commonly rely on pre-trained models \cite{hicke2023t5, fabien2020bertaa}. However, one of their significant disadvantages can be their resource-intensive nature in terms of computation or memory usage (due to the necessity of maintaining two models or important matrix parameters) and the requirement to retrain the entire model, making them challenging for modern large-scale models.\newline



\subsubsection{Decoupled Learning} is founded on the premise that pre-trained models possess a robust ability to extract general salient features from input samples. These models can serve as general feature extractors, focusing solely on feature extraction, while the task of class discrimination is handled by classifiers. This approach decouples CIL models into two distinct components: the feature extractor (pre-trained models) and the classifier \cite{belouadah2018deesil, hayes2020lifelong}. In this framework, the feature extractor is frozen after the initial training session to maintain its general feature extraction capability and prevent degradation from over-fine-tuning. Meanwhile, the classifier is permitted to update continuously throughout subsequent sessions. Decoupled learning proves highly advantageous in scenarios where a scarcity of samples from new authors leads to imbalanced datasets \cite{li2022few}. \\ 

\noindent Finally, to explore further details regarding the aforementioned approaches, please refer to the following works \cite{yan2021dynamically, zhou2022model, jodelet2023class, hu2023dense, madhavan2021incremental, li2022few}.


% Move this to the future works

% When integrated with deep metric learning, decoupled learning becomes even more powerful. It aims to transfer feature representations into distinct feature spaces, ensuring that similar samples from the same class are closely clustered while those from different classes are distinctly separated \cite{li2022few, song2023learning}. For instance, \cite{li2022few} introduced a decoupled model that seamlessly integrates various deep metric learning losses with cross-entropy loss during the initial training phase. This integration promotes both inter-class separation and intra-class compactness, thereby creating more room in the feature space for future classes. Furthermore, the effectiveness of deep metric learning within the context of AA is evident from \cite{ai2022whodunit}'s work, where a combination of cross-entropy and contrastive loss yielded promising results.\\














